CrAM: Credibility-Aware Attention Modification in LLMs for Combating Misinformation in RAG

Retrieval-Augmented Generation (RAG) can alleviate hallucinations of Large Language Models (LLMs) by referencing external documents. However, the misinformation in external documents may mislead LLMs' generation. To address this issue, we explore the task of "credibility-aware RAG", in which LLMs automatically adjust the influence of retrieved documents based on their credibility scores to counteract misinformation. To this end, we introduce a plug-and-play method named $\textbf{Cr}$edibility-aware $\textbf{A}$ttention $\textbf{M}$odification (CrAM). CrAM identifies influential attention heads in LLMs and adjusts their attention weights based on the credibility of the documents, thereby reducing the impact of low-credibility documents. Experiments on Natual Questions and TriviaQA using Llama2-13B, Llama3-8B, and Qwen1.5-7B show that CrAM improves the RAG performance of LLMs against misinformation pollution by over 20%, even surpassing supervised fine-tuning methods.

==> chapters/checklist.tex <==
\section*{Checklist}

\begin{enumerate}
\item This paper:
\begin{enumerate}
    \item  Includes a conceptual outline and/or pseudocode description of AI methods introduced. Yes.
  \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. Yes.
   \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper. Yes.
\end{enumerate}

\item Does this paper make theoretical contributions? No.






\item Does this paper rely on one or more datasets? Yes.
\begin{enumerate}
  \item A motivation is given for why the experiments are conducted on the selected datasets. Yes.
  \item All novel datasets introduced in this paper are included in a data appendix. Yes.
  \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. Yes.
  \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. Yes.
  \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. Yes.
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. NA.
  
\end{enumerate}













\item Does this paper include computational experiments? Yes.
\begin{enumerate}
  \item Any code required for pre-processing data is included in the appendix. Yes.
\item  All source code required for conducting and analyzing the experiments is included in a code appendix. Yes.
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. Yes.
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. Partial.
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. Yes.
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. Partial.
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. Yes.
\item This paper states the number of algorithm runs used to compute each reported result. Yes.
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. Yes.
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). No.
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. Yes.
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. Yes.

\end{enumerate}



\end{enumerate}

==> chapters/ethics_statement.tex <==
\section*{Ethics Statement}
In our experiments, we use gpt-3.5-turbo-0125 to generate misinformation. We want to emphasize that we generate this misinformation solely for research purposes, and we will not use it for any other purpose ourselves. Additionally, we do not encourage anyone to use this misinformation for any other purpose. 

==> chapters/limitation.tex <==
\section*{Limitations}
This work has several limitations that we aim to address in the future. 
% First, we use a constant set of heads for modification for all questions, and the results in Section \ref{sec:data size impact} indicate that the number of data points has a minor impact on the final model performance. 
First, we identify a fixed set of attention heads for attention weight modification for all questions. 
Despite Section \ref{sec:data size impact} indicating the robustness of using a small dataset for influential head identification, a more effective solution is to identify specific attention heads tailored to each individual question. 
% However, an "optimal" set of heads for a specific question should improve performance. 
% Therefore, a dynamic head selection method could significantly enhance performance. 
% Second, we found that CrAM can utilize the correct information embedded in misinformation, indicating that every detail in the documents is important. 
Second, we only use the credibility scores of each document for credibility-aware RAG. 
However, LLMs actually can utilize the correct information in the misinformation document. 
% , indicating that every detail in the documents is important. 
% Thus, implementing a fine-grained credibility score at the sentence or even word level could be very beneficial. 
Thus, empowering LLMs to leverage a fine-grained credibility score at the sentence or even word level for answer generation is promising. 
% Third, CrAM has only been verified on autoregressive transformer models and has not been explored on models with different architectures, such as T5 \citep{10.5555/3455716.3455856}.
Third, we only evaluate the performance of CrAM on decoder-only LLMs, and the effectiveness of CrAM on more models with different architectures, such as T5 \citep{10.5555/3455716.3455856}, is worth exploring. 
